Learning from Algorithm Feedback: One-Shot SAT Solver Guidance with GNNs

Boolean Satisfiability (SAT) solvers are foundational to computer science, yet their performance typically hinges on hand-crafted heuristics. This work introduces Reinforcement Learning from Algorithm Feedback (RLAF) as a paradigm for learning to guide SAT solver branching heuristics with Graph Neural Networks (GNNs). Central to our approach is a novel and generic mechanism for injecting inferred variable weights and polarities into the branching heuristics of existing SAT solvers. In a single forward pass, a GNN assigns these parameters to all variables. Casting this one-shot guidance as a reinforcement learning problem lets us train the GNN with off-the-shelf policy-gradient methods, such as GRPO, directly using the solver's computational cost as the sole reward signal. Extensive evaluations demonstrate that RLAF-trained policies significantly reduce the mean solve times of different base solvers across diverse SAT problem distributions, achieving more than a 2x speedup in some cases, while generalizing effectively to larger and harder problems after training. Notably, these policies consistently outperform expert-supervised approaches based on learning handcrafted weighting heuristics, offering a promising path towards data-driven heuristic design in combinatorial optimization.

==> Figures/graph.tex <==
\begin{tikzpicture}[>=stealth, node distance=2.5cm, auto, font=\sffamily]

    % Define styles
    \tikzstyle{clsnode}=[circle, draw=black!80, fill=rwth-carmine!20, minimum size=0.7cm, inner sep=0pt]
    \tikzstyle{litnode}=[draw=black!80, fill=rwth-darkgreen!10, minimum width=0.6cm, minimum height=0.4cm, inner sep=0pt]

    % Left partition (L)
    \node[clsnode] (C1) at (0,0.75) {$C_1$};
    \node[clsnode] (C2) at (0,-0.75) {$C_2$};
    %\node[clsnode] (L3) at (0,-2) {$C_3$};

    % Right partition (R)
    \node[litnode] (T1) at (2,1.35) {$x_1$};
    \node[litnode] (F1) at (2,0.85) {$\neg x_1$};
    \draw[line width=1pt] (T1) -- (F1);

    \node[litnode] (T2) at (2,0.25) {$x_2$};
    \node[litnode] (F2) at (2,-0.25) {$\neg x_2$};
    \draw[line width=1pt] (T2) -- (F2);

    \node[litnode] (T3) at (2,-0.85) {$x_3$};
    \node[litnode] (F3) at (2,-1.35) {$\neg x_3$};
    \draw[line width=1pt] (T3) -- (F3);

    % Edges between partitions
    \draw[line width=1pt] (C1) -- (T1.west);
    \draw[line width=1pt] (C1) -- (F2.west);
    \draw[line width=1pt] (C1) -- (F3.west);

    \draw[line width=1pt] (C2) -- (F1.west);
    \draw[line width=1pt] (C2) -- (F3.west);
    
\end{tikzpicture}

==> Figures/search.tex <==
\begin{tikzpicture}[
    %>=Stealth, 
    % Node style: square with rounded corners, 7mm size
    every node/.style={
      draw,
      rectangle,
      rounded corners=2pt,
      minimum width=12mm,
      minimum height=6mm,
      align=center,
      fill=black!05,
    },
    % Edge label style: smaller boxes, smaller font
    edge label/.style={
      draw,
      rectangle,
      rounded corners=0pt,
      fill=white,
      %font=\scriptsize,
      minimum width=7mm,
      minimum height=5mm,
      inner sep=1pt,
      align=center,
      anchor=center,
    }
]

  % Root node
  \node (root) at (0,0) {$\hat{x} = {\arg\!\max}_x \  {\color{green!60!black}w(\!x\!)} \! \cdot \! \textsc{Score}(\!x\!)$};

  % "..." above the root (suggesting more tree above)
  \draw[<-,thick,densely dotted] (root.north) -- ++(0.0,0.3);

    % Children placed below-left and below-right relative to root
    \node (left)  [below left=1.5cm and 1.0cm of root.center] {$\cdots$};
    \node (right) [below right=1.5cm and 1.0cm of root.center] {$\cdots$};
    
  % Edges from root to children, with a small box labeled "1"
  \draw[->,thick] (root) -- node[edge label, midway, fill=rwth-blue!10, draw=rwth-blue!70]{$\neg\hat{x}$} (left);
  \draw[->,thick] (root) -- node[edge label, midway, fill=rwth-red!10, draw=rwth-red!70]{$\hat{x}$} (right);

  % "..." below the left child (suggesting more subtree below)
  \draw[->,thick,densely dotted] (left.center) -- ++(-0.4,-0.6);
  \draw[->,thick,densely dotted] (left.center) -- ++(0.4,-0.6);

  % "..." below the right child
  \draw[->,thick,densely dotted] (right.center) -- ++(-0.4,-0.6);
  \draw[->,thick,densely dotted] (right.center) -- ++(0.4,-0.6);

  \node (left)  [below left=1.5cm and 1.0cm of root.center] {$\cdots$};
  \node (right) [below right=1.5cm and 1.0cm of root.center] {$\cdots$};  
\end{tikzpicture}

